Kronecker states: a powerful source of multipartite maximally entangled states in quantum information

In quantum information theory, maximally entangled states, specifically locally maximally entangled (LME) states, are essential for quantum protocols. While many focus on bipartite entanglement, applications such as quantum error correction and multiparty secret sharing rely on multipartite entanglement. These LME states naturally appear in the invariant subspaces of tensor products of irreducible representations of the symmetric group $S_n$, called Kronecker subspaces, whose dimensions are the Kronecker coefficients. A Kronecker subspace is a space of multipartite LME states that entangle high-dimensional Hilbert spaces. Although these states can be derived from Clebsch-Gordan coefficients of $S_n$, known methods are inefficient even for small $n$. A quantum-information-based alternative comes from entanglement concentration protocols, where Kronecker subspaces arise in the isotypic decomposition of multiple copies of entangled states. Closed forms have been found for the multiqubit $W$-class states, but not in general. This thesis extends that approach to any multiqubit system. We first propose a graphical construction called W-state Stitching, where multiqubit entangled states are represented as tensor networks built from $W$ states. By analyzing the isotypic decomposition of copies of these graph states, corresponding graph Kronecker states can be constructed. In particular, graph states of generic multiqubit systems can generate any Kronecker subspace. We explicitly construct bases for three- and four-qubit systems and show that the W-stitching technique also serves as a valuable tool for multiqubit entanglement classification. These results may open new directions in multipartite entanglement resource theories, with bipartite and tripartite $W$ states as foundational elements, and asymptotic analysis based on Kronecker states.

==> Chapters/Stitching.tex <==
\label{Chapter4}
In this section, we present a graphical method for constructing generic qubit states using $W_3$ states and bipartite states. The idea of representing quantum elements in a graphical notation is not new, for example, the very well known approach of graph states \cite{Graphstates} uses vertices to represent qubits and edges to represent the interaction between them, and it has a broad range of applications in quantum error correction and quantum computation. Another very relevant graphical method is the  $ZW$ calculus \cite{ZW}, which we learned about during the final stage of this investigation. In this method, processes are represented by diagrams, where each part of the system is represented by a line that can interact with other elements or lines, and the nature of interactions is given by the elements present in each path of each line. This construction is very rich and there are symbols and rules for every possible action in the quantum system. \\

\noindent In ZW calculus, $W$ states are special elements as they are for us, and some results that we present here were also obtained in this construction, however, the elements that we use in our construction exploit the symmetries of $W$ states to make powerful observations. There is also a difference in the way that our graphs must be read, allowing us to understand graphs as states and facilitating SLOCC classification, in contrast with $ZW$ calculus, where the graphs are thought as directional processes.\\

\noindent  We begin this chapter by introducing the stitching procedure and the graphical notation that will be utilized. This notation was adapted to the used in $ZW$ calculus to avoid confusion for readers who are familiar with the method. Subsequently, we explore a graphical interpretation of the symmetries within the $W_3$ state, which we refer to as \textit{Pushing parameters}, which is the most remarkable difference with the $ZW$ calculus. Applying this technique allows us to simplify the various graphs that can be generated, reducing the parameters that are relevant under SLOCC classification for each graph. We explore this construction for the cases of two, three and four qubits, finding graphs that represent states in all the possible SLOCC classes in both.\\

\noindent Moreover, in \nameref{Invariants} we illustrate how this construction enables a clear visualization of the invariants, which we leverage to explicitly build a set of invariants for two, three and four-qubit systems, and  more impressively, to build $17$ elements corresponding to a possible invariant basis for a $5$-qubit system. 

\section{The Stitching Procedure}
\textit{Stitching} is a method for constructing multiqubit states using graph states with two building blocks: the $W_3$ state as kets, and bipartite qubit states in general entangled as bras. The unnormalized $W_3$ state is given by
\begin{equation}
\ket{W_3} =\ket{100}+\ket{010}+\ket{001}.
\end{equation}
The bipartite state, from now on, the stitch, in general, can be written as
\begin{equation*}
\bra{\varsigma}= \varsigma_{00}\bra{00}+\varsigma_{01}\bra{01}+\varsigma_{10}\bra{10}+\varsigma_{11}\bra{11}.
\end{equation*}
This state can also be written as
\begin{equation*}
    \bra{\varsigma}= \bra{\phi^{+}} I\otimes  \bm{\varsigma} , \quad  
     \bm{\varsigma} := \left( \begin{array}{cc}
          \varsigma_{00}&\varsigma_{01}  \\
         \varsigma_{10} & \varsigma_{11}
     \end{array}\right). 
\end{equation*}
By restricting the matrix $\bm{\varsigma}$ to unit determinant, i.e., $\varsigma_{11}=\frac{1+\varsigma_{01}\varsigma_{10}}
{\varsigma_{00}}$, which corresponds to multiplying a global factor by the state, the stitch can be written as
\begin{equation}
    \bra{\varsigma} = \bra{\phi^{+}} \mathcal{A} \left(\varsigma_{10}/\varsigma_{00} \right) \otimes u( \varsigma_{00}, \varsigma_{01}),
    \label{eq:stitch1}
\end{equation}
where $u$ and $\mathcal{A}$ are upper diagonal matrices with unit determinant, according to 
\begin{equation*}
    u(v,w):= \left( \begin{array}{cc}
       v  & w \\
        0 & 1/v
    \end{array}
     \right) , \quad \mathcal{A}(w):=u(1,w),
\end{equation*}
then $\mathcal{A}$ and $u$ operate in the different parts of the bipartite state. When the stitch has a 0 in the last entry i.e., $\varsigma_{11}=0$, then the stitch must be parametrized as:
\begin{equation*}
     \bm{\varsigma} := \left( \begin{array}{cc}
\varsigma_{00}&\varsigma_{01}=-\frac{1}{\varsigma_{10} } \\
       \varsigma_{10} & 0
     \end{array}\right)
\end{equation*}
and then it can be written again as in equation \eqref{eq:stitch1}. Another case is when $\varsigma_{00}=0$, then the unit determinant matrix is
\begin{equation*}
\bm{\varsigma^{*}}=\left( \begin{array}{cc}
      0 &\varsigma_{01}  \\
          \frac{1}{\varsigma_{01}} & \varsigma_{11}
     \end{array}\right),
\end{equation*}
and the state can be written as
\begin{equation*}    \bra{\varsigma^{*}}=\bra{\phi^{+}} I \otimes X u(1/ \varsigma_{01},\varsigma_{11}) =\bra{\psi^{+}} I \otimes  u(1/ \varsigma_{01},\varsigma_{11}),
\end{equation*}
with $X$ the Pauli operator. We introduce another kind of upper matrix
\begin{equation*}
    \mathcal{B}(v):= u(v,0),
\end{equation*}
which will be useful later. Then we define a graphical notation for each element:
\begin{equation*}
    \mathcal{B}(v)   : \tikz {\filldraw [color=black!, fill=white!] (0,0) circle[radius=3pt];
    \node[above=1mm] {$v$} (0.1,0.2);}, \quad  \mathcal{A}(w): \tikz{
   \draw [\rao]
           (0,0) -- (1,0) ; \draw (0.9,0.3) node {$w$}
   }
   \quad  u(v,w): \tikz{
   \draw  [\rac]           (0,0) -- (1,0)  ; \draw (0.9,0.3) node {$(v,w)$};
  } = \tikz{
   \draw  [\rao]           (0,0) -- (1,0) ;
   \filldraw [color=black!, fill=white!] (0.6,0) circle[radius=3pt];
   \draw (1.1,0.3) node {$w/v$};
   \draw (0.6,0.3) node {$v$};}.
\end{equation*}
With this, we can introduce a graphical notation for the two cases of a bipartite state:
\begin{equation*}
   \bra{\varsigma} = \begin{tikzpicture} [basel={-1.5},every node/.style={scale=0.6}]
       \draw [\lao \rac]            (0,0) -- (2,0) ;   
   \draw (0,0.3) node {$\varsigma_{10}/\varsigma_{00}$};
   \draw (2,0.3) node {$(\varsigma_{00},\varsigma_{01})$};
   \end{tikzpicture}, \quad \bra{\varsigma^*} =\begin{tikzpicture}
        [basel={-1.5},every node/.style={scale=0.6}]
        \draw [\rac]        (0,0) -- (2,0) ;  ;\draw[markxi={0.5}] (0,0)--(2,0) ;
        \draw (2,0.3) node {$(1/\varsigma_{01},\varsigma_{11})$};         \end{tikzpicture},
\end{equation*}
where an empty line refers to the $\bra{\phi^+}$ state and the line with $\bullet$ refers to the $\bra{\psi^{+}}$ state. Note how the two cases from equation \eqref{eq:stitch1} can be represented with the first diagram. We now introduce a graphical notation for the $W$ state: 
\begin{equation*}
    \ket{W_3}=\begin{tikzpicture}[basel={-.5}]
  \draw[markx={1}] (0,0) to (0.5,0);
  \draw (0.5,0) to (1,0.5);
  \draw (0.5,0) to (1,-0.5);
  \draw (1,0.7) node {$B$};
  \draw (1,-0.7) node {$C$};
  \draw (-0.3,0) node {$A$};
\end{tikzpicture}, 
\end{equation*}
 The idea behind the stitching process is to build a graph state $\ket{G}$ by taking the tensor product of $w$ $\ket{W_3}$ states and \emph{stitch} them using projection with  a number $s$ of  $\bra{\varsigma}$ states, explicitly

\begin{equation}    \ket{G}=\bigotimes_{i=1}^{s}\bra{\varsigma^{i}}\bigotimes_{i=1}^{w}\ket{W_3},
\label{eq:GraphConstruction}
\end{equation}
where the contractions between $\bra{\varsigma}$ and $\ket{W_3}$ are determined by the topology of the graph state $G$. The simplest example is shown in Figure \ref{fig:Tree4}, where two $W_3$ states are stitched with a two-particle state $\bra{\varsigma^{}}$ to obtain a four-qubit state. Notice that only uncontracted parties are labeled.\\

\begin{figure}[h!]
\centering
%\includegraphics[scale=0.35]{Tree4.png}
\begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]  
  \draw[markx={1}] (-0.5,0) to (-1,0);
  \draw (-1,0) to (-1.5,0.5);
  \draw (-1,0) to (-1.5,-0.5);
  \draw (-1.7,0.7) node {$A$};
  \draw (-1.7,-0.7) node {$B$};
  \draw (-0.5,-0.2) node {$E$};
    \draw[\lao \rac ] (0,0) -- (2,0);
 \draw[markx={1}] (2.5,0) to (3,0);
  \draw (3,0) to (3.5,0.5);
  \draw (3,0) to (3.5,-0.5);
  \draw (3.5,0.7) node {$C$};
  \draw (3.5,-0.7) node {$D$};
  \draw (2.2,-0.2) node {$F$};
\end{tikzpicture} = 
\begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]  
  \draw [markx={0}](-1,0) to (-1.5,0.5);
  \draw (-1,0) to (-1.5,-0.5);
  \draw (-1.7,0.7) node {$A$};
  \draw (-1.7,-0.7) node {$B$};
    \draw[\lao \rac ] (-1,0) -- (0,0);
  \draw[markx={0}] (0,0) to (0.5,0.5);
  \draw (0,0) to (0.5,-0.5);
  \draw (0.5,0.7) node {$C$};
  \draw (0.5,-0.7) node {$D$};
\end{tikzpicture}
\caption{Graph in tree form, stitching two $W_3$ states with a stitch $\varsigma$, to obtain a four-qubit state. The contraction occurs in the E and F parties of the $\ket{W_3}$ states which are not labeled in the resulting $\ket{G}$ state.}
\label{fig:Tree4}
\end{figure}

\noindent The state obtained in the stitching procedure depends on the structure of the graph and the parameters of the stitch. Such graphs allow inner loops and as much structure as desired. The number of qubits in the resultant state is given by:
\begin{equation}
N=3w-2s.
\label{eq:Numberofparts}
\end{equation}
 For example, in Figure \ref{fig:GenStitch}, a graph where $6$ $\ket{W_3}$ states are stitched using $7$ $\bra{\varsigma}$ states results in a $6\cdot 3-2\cdot7=4$ qubit state.

\begin{figure}[h!]
\centering
\scalebox{1.3}{
     \begin{tikzpicture}[baseline={([yshift=-.5ex]current bounding box.center)},every node/.style={scale=0.6}]
    \draw[\lao \rac](1,1) -- (0,0);
     \draw[\lao \rac](1,-1) -- (0,0);
      \draw[\lao \rac](1,1) -- (1.5,0.5);
       \draw[\lao \rac](1,-1) -- (1.5,-0.5);
    \draw[\lao \rac](1.5,-0.5) -- (2,0);
    \draw[markxi={0}](1.5,0.5) -- (2,0);
    \draw[markxi={0}](1.5,-0.5) -- (2,0);
    \draw[\lao \rac](1.5,0.5) -- (2,0);
      \draw[\lao \rac](1.5,0.5) -- (1.5,-0.5);
\draw[markx={1}](-0.5,0) -- (0,0);
\draw[markx={0}](2,0) -- (2.5,0);
\draw[markx={0}](1,1) -- (0.5,1.5);
     \draw[markx={0}](1,-1) -- (0.5,-1.5);
     \draw (-0.5,0.3) node {$A$};
      \draw (0.5,1.3) node {$B$};
       \draw (2.5,0.3) node {$C$};
        \draw (0.5,-1.3) node {$D$};
    \end{tikzpicture}}
%\includegraphics[scale=0.5]{GenStitch.png}
\caption{An example of the Stitching procedure, where 6 $W_3$ states are stitched by 7 $\varsigma$ states, leaving $4$ free edges, corresponding to a four-qubit state.}
\label{fig:GenStitch}
\end{figure}

\subsection*{SLOCC equivalent graphs}

In quantum physics, the SLOCC operations define whether one state can be inter-converted to another one or not, dividing the Hilbert space into different orbits with different entanglement properties, due to SLOCC operations cannot create entanglement. In the graphical notation, actions over outer edges correspond to SLOCC operations, however, we can see that some inner actions will lead to the same SLOCC orbits, for example, consider the next two graph states: 
\begin{equation*}
 \begin{tikzpicture}[baseline={([yshift=-.5ex]current bounding box.center)},every node/.style={scale=0.6}] 
 \foreach \n in {1,...,3}{
        \node at ($(0,0)+({240+\n*360/3}:0.7cm) $)(n\n) {};
        \draw (0,0)--(n\n); }
    \draw[\lao-] (0,0) -- (1,0);
   \foreach \n in {1,...,3}{
        \node at ($(1,0)+({60+\n*360/3}:0.7cm) $)(n\n) {};
        \draw[markx={0},markx={1}] (0,0) to (1,0); 
        \draw (1,0)--(n\n); }
        \draw (-0.5,0.5) node {$A$};
         \draw (-0.5,-0.5) node {$B$};
         \draw(0,0.3) node {$w$};
         \draw (0.8,0.3) node {$v$};
         \ball{(0.8,0)};
 \draw (1.5,0.5) node {$C$};
  \draw (1.5,-0.5) node {$D$};
\end{tikzpicture} = \frac{1}{v}\ket{0000} +v w  \ket{00}\ket{W_2}+v\ket{W_2}\ket{W_2}, 
\end{equation*}
\begin{equation*}
 \begin{tikzpicture}[baseline={([yshift=-.5ex]current bounding box.center)},every node/.style={scale=0.6}]  
 \foreach \n in {1,...,3}{
        \node at ($(0,0)+({240+\n*360/3}:0.7cm) $)(n\n) {};
        \draw (0,0)--(n\n); }
    \draw (0,0) -- (1,0);
   \foreach \n in {1,...,3}{
        \node at ($(1,0)+({60+\n*360/3}:0.7cm) $)(n\n) {};
        \draw[markx={0},markx={1}] (0,0) to (1,0); 
        \draw (1,0)--(n\n); }
        \draw (-0.5,0.5) node {$A$};
         \draw (-0.5,-0.5) node {$B$};
 \draw (1.5,0.5) node {$C$};
  \draw (1.5,-0.5) node {$D$};
\end{tikzpicture} = \ket{0000} +\ket{W_2}\ket{W_2}.
\end{equation*}
They both belong to the same SLOCC orbit, namely $L_{a00_2} (L_{abc_2} , b=c=0)$ in Verstraete classification \cite{Verstraete}. The first one can be obtained from the second one with the next SLOCC operation:
\begin{equation*}
v \cdot \begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]  
 \foreach \n in {1,...,3}{
        \node at ($(0,0)+({240+\n*360/3}:0.7cm) $)(n\n) {};
        \draw (0,0)--(n\n); }
    \draw (0,0) -- (1,0);
   \foreach \n in {1,...,3}{
        \node at ($(1,0)+({60+\n*360/3}:0.7cm) $)(n\n) {};
         \draw[markx={0},markx={1}] (0,0) to (1,0); 
        \draw (1,0)--(n\n); }
        \draw (-0.5,0.5) node {$A$};
         \draw (-0.5,-0.5) node {$B$};
 \draw (1.5,0.5) node {$C$};
  \draw (1.5,-0.5) node {$D$};
  \ball{(1.1,0.2)};
  \ball{ (1.1,-0.2)};
  \draw[\rao] (-0.3,0.5) to (0,0);
  \draw (0,0.3) node {$w$};
  \draw (1,0.4) node {$1/v$};
    \draw (1,-0.4) node {$1/v$};
\end{tikzpicture} =\begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]  
 \foreach \n in {1,...,3}{
        \node at ($(0,0)+({240+\n*360/3}:0.7cm) $)(n\n) {};
        \draw (0,0)--(n\n); }
    \draw[\lao-] (0,0) -- (1,0);
   \foreach \n in {1,...,3}{
        \node at ($(1,0)+({60+\n*360/3}:0.7cm) $)(n\n) {};
        \draw (1,0)--(n\n); }
          \draw[markx={0},markx={1}] (0,0) to (1,0); 
        \draw (-0.5,0.5) node {$A$};
         \draw (-0.5,-0.5) node {$B$};
         \draw(0,0.3) node {$w$};
         \draw (0.8,0.3) node {$v$};
         \ball{(0.8,0)};
 \draw (1.5,0.5) node {$C$};
  \draw (1.5,-0.5) node {$D$};
\end{tikzpicture}
\end{equation*}
This simple example shows how some of the information given by the stitches can be translated into SLOCC operations. In more complex cases, as the graph in Figure \ref{fig:GenStitch}, identifying the relevant information will prove to be necessary as there are $21$ complex parameters in the stitches, and in four qubits, the most general SLOCC class depends only on 3 complex parameters. In the next section, we present a supplementary tool that allows us to identify the relevant parameters in the stitching procedure.
\section{Pushing parameters}
The $W_3$ state has an interesting symmetry in terms of $u$ operations that can be used to switch between inner and outer actions. In general, the action of $u$ in one of the parts can be exchanged for actions in the other two parts as:
\begin{equation}
    u(v,w) \otimes I \otimes I \ket{W} = I \otimes u(1/v ,w_1) \otimes u(1/v,w_2) \left( v\ket{W} \right)
    \label{eq:Wstabilizer},
\end{equation}
where $w_1+w_2=w$. In most cases, we will set $w_1=w,w_2=0$. This property is understood as that we \textit{Pushed} the action in one of the parts to the other two. Graphically, the property in Eq \eqref{eq:Wstabilizer} is:
\begin{equation}
   \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]]
   \draw [\rac]            (0,0) -- (0.5,0) ;
   \draw[markx={1}] (1,0.5) -- (0.5,0);
  \draw (1,-0.5) -- (0.5,0);
   \draw (0.3,0.3) node  {$(v,w)$};
	 \end{tikzpicture} \equiv v\cdot  \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]]
   \draw  (0,0) -- (0.5,0) ;
  \draw [\rac](1,0.5) -- (0.5,0);
   \draw[markx={1}]  (1,-0.5) -- (0.5,0);
   \ball{(0.8,-0.3)}
   \draw (0.7,0.7)  node {$(1/v,w)$};
   \draw (0.7,-0.7) node {$1/v$};
\end{tikzpicture}.
  \label{eq:rule1}
\end{equation}
From now on, we will use the symbol ``$\equiv$'' to denote exact equality and ``$=$'' when some proportionality factor is omitted. Note that $\mathcal{A}$ and $\mathcal{B}$ are just special cases of $u$, so the next properties are also true:
\begin{equation}
     \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
   \draw[markx={1}]  (0.5,0) -- (1,0) ;
   \ball{(0.7,0)};
   \draw (1.5,0.5) -- (1,0);
   \draw (1.5,-0.5) -- (1,0);
   \draw (0.7,0.3) node {$v$};
\end{tikzpicture} = \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
   \draw[markx={1}]   (0.5,0) -- (1,0) ;
   \draw (1.5,0.5) -- (1,0);
   \draw (1.5,-0.5) -- (1,0);
   \ball{ (1.3,0.3) }
  \ball{(1.3,-0.3) }   
   \draw (1.3,0.7) node {$1/v$};   
   \draw (1.3,-0.7) node {$1/v$};
\end{tikzpicture} , \quad  \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
   \draw [\rao]            (0.5,0) -- (1,0) ;
   \draw[markx={1}]  (1.5,0.5) -- (1,0);
   \draw (1.5,-0.5) -- (1,0);
   \draw (0.8,0.3) node {$w$};
\end{tikzpicture} \equiv \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
   \draw [markx={1}]  (0.5,0) -- (1,0) ;
   \draw [\rao](1.5,0.5) -- (1,0);
   \draw (1.5,-0.5) -- (1,0);
    \draw (1.1,0.5) node {$w$};
\end{tikzpicture}.
   \label{eq:rule2}
\end{equation}
 Three more properties based on the algebras of $\mathcal{B}$ and $u$ will help with the pushing.
 \begin{equation}
\begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
     \draw (0,0)-- (1,0);
     \ball{(0.4,0)};
     \ball{(0.7,0)};
     \draw (0.4,0.3) node {$v_1$};
     \draw (0.7,0.3) node {$v_2$};
\end{tikzpicture} \equiv
\begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
     \draw  (0,0)-- (1,0);
     \ball{(0.5,0)};
     \draw (0.4,0.3) node {$v_1v_2$};
\end{tikzpicture} , \quad \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
     \draw[\rao] (0,0)-- (0.7,0);
     \draw[\rao] (0.7,0)-- (1,0);
     \draw (0.5,0.3) node {$w_1$};
     \draw (1,0.3) node {$w_2$};
\end{tikzpicture} \equiv\begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
     \draw[\rao] (0,0)-- (1,0);
     \draw (0.7,0.3) node {$w_1+w_2$};
\end{tikzpicture}  ,\quad \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
     \draw[\rac] (0,0)-- (1,0);
     \draw (0.7,0.3) node {$(v,w)$};
\end{tikzpicture}  \equiv\begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
     \draw[\rao] (0,0)-- (1,0);
     \ball{(0.6,0)};
     \draw (1,0.3) node {$w/v$};
      \draw (0.5,0.3) node {$v$};
\end{tikzpicture}=\begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
     \draw[\rao] (0,0)-- (0.6,0);
     \draw (0.6,0)--(1,0);
     \ball{(1,0)};
     \draw (1,0.3) node {$v$};
      \draw (0.5,0.3) node {$wv$};
\end{tikzpicture}.
   \label{eq:rule3}
\end{equation}  
 Balls can be moved through lines, but when there is a $\bullet$ they invert the argument, and arrows can be flipped in $\bullet$ lines:
\begin{equation}
   \tikz {\draw (0,0)--(1,0);\filldraw [color=black!, fill=white!] (0.2,0) circle[radius=3pt];\draw (0.2,0.3) node {$v$};} \equiv \tikz {\draw (0,0)--(1,0);\filldraw [color=black!, fill=white!] (0.8,0) circle[radius=3pt];\draw (0.8,0.3) node {$v$};}, \begin{tikzpicture}[basel={-2}]    
\draw[markx={0.5}] (0,0)--(1,0);\ball{(0.2,0)} ;\draw (0.2,0.3) node {$v$};\end{tikzpicture} \equiv \begin{tikzpicture}[basel={-2}]
\draw[markx={0.5}] (0,0)--(1,0);\ball{(0.8,0)} ;\draw (0.8,0.3) node {$1/v$};\end{tikzpicture},   \begin{tikzpicture}[basel={-1.8},every node/.style={scale=0.6}]       
   \draw[\rac]   (0,0)--(1,0);\draw[markxi={0.5}] (0,0) -- (1,0) ;
    \draw (1,0.3) node {$(v,w)$}
   ;\end{tikzpicture}\equiv \begin{tikzpicture}[basel={-2.2},every node/.style={scale=0.6}]    
   \draw[-\lac] (1,0)--(0,0);\draw[markxi={0.5}]   (1,0)--(0,0);
   \draw (0,0.3) node {$(1/v,w)$};
   \end{tikzpicture}.
   \label{eq:rule4}
\end{equation}
It will be common to have some arrows and $\bullet$ acting on each other in different directions. From their algebras we can get:
\begin{equation}
    \begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]
    \draw[\rac](0,0) to (1,0);
    \draw[\lac-](1,0) to (2,0);
    \draw (0.5,0.3) node {$(v_1,w_1)$};
    \draw (1.5,0.3) node {$(v_2,w_2)$};
    \end{tikzpicture} \equiv \begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]
        \draw[\lao \rac](0,0) to (2,0);
         \draw (0,0.3) node {$\frac{v_2}{w_1(v_1v_2+w_1w_2)}$};
    \draw (2,0.3) node {$(v_1v_2+w_1w_2 ,v_1/w_2)$};
    \end{tikzpicture} , \quad \begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]
        \draw[\rac](0,0) to (1,0);
        \draw[markx={0.5}] (1,0) to (2,0);
        \draw (0.5,0.3) node {$(v,w)$};
    \end{tikzpicture} \equiv -i \cdot \begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]
        \draw[\lao \rac](0,0) to (2,0);
        \draw (0,0.3) node {$1/vw$};
        \draw (2,0.3) node {$(iw,iv)$};
    \end{tikzpicture}
    \label{eq:rule5}
\end{equation}
The cases with white arrows can be obtained by replacing $v=1$. Equations \eqref{eq:rule1}\eqref{eq:rule2}\eqref{eq:rule3}\eqref{eq:rule4} and \eqref{eq:rule5} are the basic rules of pushing, however we explore the construction in \nameref{Appendix03} how some more rules can be obtained from the different constructions. Here we summarize those results as the set of Stitching and Pushing rules.

 \section{Stitching and Pushing Rules}
 \label{Rules}
 \begin{enumerate}
     \item Stitch-Arrows equivalence:
     \begin{equation}
     \bra{\varsigma}\equiv
  \begin{tikzpicture}  
  \draw[\lao \rac] (0,0) to (1,0);
    \end{tikzpicture}, \quad \bra{\varsigma^*}\equiv
    \begin{tikzpicture}
         \draw[ \rac] (0,0) to (1,0);
         \draw[markxi={0.5}] (0,0) to (1,0);
    \end{tikzpicture},
\end{equation}
where $\varsigma^{*}$ corresponds to cases where $\varsigma_{00}=0$. 
\item Multiplication rules:
\begin{equation}
    \begin{tikzpicture}[basel={-2}]
        \draw(0,0) to (1,0); 
        \draw (0.3,0.3) node {$v_1$};
        \draw (0.7,0.3) node {$v_2$};
        \ball{(0.3,0)};
        \ball{(0.7,0)};       
    \end{tikzpicture}\equiv\begin{tikzpicture}[basel={-2}]
        \draw(0,0) to (1,0); 
        \draw (0.5,0.3) node {$v_1v_2$};
        \ball{(0.5,0)};
    \end{tikzpicture} , \quad \begin{tikzpicture}[basel={-2}]
        \draw[\rao](0.6,0) to (1,0);
        \draw[\rao](0,0) to (0.6,0);
        \draw (0.5,0.3) node {$w_1$};
        \draw (1,0.3) node {$w_2$};
    \end{tikzpicture} \equiv\begin{tikzpicture}[basel={-2}]
        \draw[\rao](0,0) to (1,0);
         \draw (1,0.3) node {$w_1+w_2$};
    \end{tikzpicture} , \quad \begin{tikzpicture}[basel={-2}]
        \draw[\rac](0,0) to (1,0);
        \draw (1,0.3) node {$(v,w)$};
    \end{tikzpicture} \equiv\begin{tikzpicture}[basel={-2}]
        \draw[\rao](0,0) to (1,0);
        \ball{(0.5,0)}
        \draw (0.5,0.3) node {$v$};
        \draw (1,0.3) node {$w/v$};
\end{tikzpicture}\equiv\begin{tikzpicture}[basel={-2}]
        \draw[\rao](0,0) to (0.5,0);
        \draw(0.5,0) to (1,0);
        \ball{(1,0)}
        \draw (0.2,0.3) node {$vw$};
        \draw (1,0.3) node {$v$};
    \end{tikzpicture}.
\end{equation}
\item Movement rules:
\begin{equation}
    \begin{tikzpicture}[basel={-2}]
        \draw(0,0) to (1,0); 
        \draw (0,0.3) node {$v$};
        \ball{(0,0)};      
    \end{tikzpicture}\equiv\begin{tikzpicture}[basel={-2}]
        \draw(0,0) to (1,0); 
        \draw (1,0.3) node {$v$};
        \ball{(1,0)};  
    \end{tikzpicture}, \quad \begin{tikzpicture}[basel={-2}]
        \draw[markx={0.5}](0,0) to (1,0); 
        \draw (0,0.3) node {$v$};
        \ball{(0,0)};      
    \end{tikzpicture}\equiv\begin{tikzpicture}[basel={-2.2}]
        \draw[markx={0.5}](0,0) to (1,0); 
        \draw (1,0.3) node {$1/v$};
        \ball{(1,0)};  
    \end{tikzpicture} , \quad \begin{tikzpicture}[basel={-2}]
        \draw[\lac-](0,0) to (1,0);
        \draw[markxi={0.5}](0,0) to (1,0);
        \draw (0,0.3) node {$(v,w)$};  
    \end{tikzpicture}\equiv\begin{tikzpicture}[basel={-2.2}]
        \draw[\rac](0,0) to (1,0);
          \draw[markxi={0.5}](0,0) to (1,0);
        \draw (1,0.3) node {$(1/v,w)$};
    \end{tikzpicture}.
    \end{equation}
\item Pushing rules:
    \begin{equation}
        \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
        \draw[\rac](0,0) to (0.5,0);
        \draw[markx={0}] (0.5,0) to (1,0.5);
        \draw (0.5,0) to (1,-0.5);
        \draw (0.2,0.3) node {$(v,w)$};
    \end{tikzpicture}\equiv v\cdot \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
        \draw(0,0) to (0.5,0);
        \draw[\lac-] (0.5,0) to (1,0.5);
        \draw[markx={0}] (0.5,0) to (1,-0.5);
        \ball{(0.8,-0.3)};
        \draw (0.5,0.6) node {$(1/v,w)$};
         \draw (0.8,-0.7) node {$(1/v)$};
    \end{tikzpicture} , \quad \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
        \draw(0,0) to (0.5,0);
        \draw [markx={0}](0.5,0) to (1,0.5);
        \draw (0.5,0) to (1,-0.5);
        \ball{(0.3,0)};
        \draw (0.3,0.3) node {$v$};
    \end{tikzpicture} \equiv v\cdot\begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
        \draw(0,0) to (0.5,0);
        \draw[markx={0}] (0.5,0) to (1,0.5);
        \draw (0.5,0) to (1,-0.5);
        \ball{(0.8,0.3)};
        \ball{(0.8,-0.3)};
         \draw (0.8,0.6) node {$1/v$};
          \draw (0.8,-0.6) node {$1/v$};
    \end{tikzpicture} , \quad
        \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
        \draw[\rao](0,0) to (0.5,0);
        \draw[markx={0}] (0.5,0) to (1,0.5);
        \draw (0.5,0) to (1,-0.5);
        \draw (0.2,0.3) node {$w$};
    \end{tikzpicture}\equiv\begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
        \draw(0,0) to (0.5,0);
        \draw[\lao-] (0.5,0) to (1,0.5);
        \draw[markx={0}] (0.5,0) to (1,-0.5);
        \draw (0.5,0.3) node {$w$};
    \end{tikzpicture} .
    \end{equation}
    \item Arrow-Arrow, Arrow-$\bullet$ operations:
    \begin{equation}
    \begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]
    \draw[\rac](0,0) to (1,0);
    \draw[\lac-](1,0) to (2,0);
    \draw (0.5,0.3) node {$(v_1,w_1)$};
    \draw (1.5,0.3) node {$(v_2,w_2)$};
    \end{tikzpicture} \equiv \begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]
        \draw[\lao \rac](0,0) to (2,0);
         \draw (0,0.3) node {$\frac{v_2}{w_1(v_1v_2+w_1w_2)}$};
    \draw (2,0.3) node {$(v_1v_2+w_1w_2 ,v_1/w_2)$};
    \end{tikzpicture} , \quad \begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]
        \draw[\rac](0,0) to (1,0);
        \draw[markx={0.5}] (1,0) to (2,0);
        \draw (0.5,0.3) node {$(v,w)$};
    \end{tikzpicture} \equiv -i \cdot \begin{tikzpicture}[basel={-.5},every node/.style={scale=0.6}]
        \draw[\lao \rac](0,0) to (2,0);
        \draw (0,0.3) node {$1/vw$};
        \draw (2,0.3) node {$(iw,iv)$};
    \end{tikzpicture}
\end{equation}
\item One Quibt definitions:
\begin{equation}
\ket{1}=  \begin{tikzpicture}[basel={-.6}]
     \qubitl{(0,0)} ;
      \draw(-0.5,0) to (-0.25,0);
   \end{tikzpicture} , \quad \ket{0}=\begin{tikzpicture}[basel={-.6}]
      \qubitl{(0,0)} ;
      \draw[markx={0.5}](-0.5,0) to (-0.25,0);
   \end{tikzpicture}.
\end{equation}
    \item W rotation rule:
    \begin{equation}
    \begin{tikzpicture}[basel={-0.5}]
   \draw (0,0) -- (0.5,0) ; 
   \draw (0.5,0) -- (0,0) ;
   \draw (-0.25,0.25) -- (0,0);
   \draw (-0.25,-0.25) -- (0,0);\draw (0.75,0.25) -- (0.5,0);
   \draw (0.72,-0.25) -- (0.5,0);\draw[markxi={0},markxi={0.5},markxi={1}] (0,0)--(0.5,0) ;
   \draw (-0.35,0.25) node{$1$};
    \draw (-0.35,-0.25) node{$2$};
     \draw (0.85,0.25) node{$3$};
      \draw (0.85,-0.25) node{$4$}; 
\end{tikzpicture} \equiv \begin{tikzpicture}[basel={-0.5}]
   \draw (0,0) -- (0.25,0.25) ; 
   \draw (-0.25,0.25) -- (0,0) ;
   \draw (0,0) -- (0,-0.5);
   \draw (0,-0.5) -- (0.25,-0.75);\draw (0,-0.5) -- (-0.25,-0.75);
  \draw[markxi={0},markxi={0.5},markxi={1}] (0,0)--(0,-0.5) ;
   \draw (-0.35,0.25) node{$1$};
    \draw (-0.35,-0.75) node{$2$};
     \draw (0.35,0.25) node{$3$};
      \draw (0.35,-0.75) node{$4$};
\end{tikzpicture}
\label{eq:rule7}
\end{equation}
\item Loop rules:
\begin{equation}
      \begin{tikzpicture}[basel={-0.5}]
        \draw[markx={1}] (0,0) to (0.5,0);
       \draw[markx={0.9}] (0.5,0)to[bend left=70] (1.5,0);
         \draw (0.5,0)to[bend right=70] (1.5,0);
            \ball{(1,0.25)};
    \end{tikzpicture} \equiv \left( \frac{1+v^2}{v}\right) \cdot \begin{tikzpicture}[basel={-.6}]
      \qubitl{(0,0)} ;
      \draw[markx={0.5}](-0.5,0) to (-0.25,0);
   \end{tikzpicture} , \quad  \begin{tikzpicture}[basel={-0.5}]
        \draw [markx={1}](0,0) to (0.5,0);
       \draw[markxo={0.9}{0.5}] (0.5,0)to[bend left=70] (1.5,0);
         \draw (0.5,0)to[bend right=70] (1.5,0);
    \end{tikzpicture} \equiv \varnothing.
\end{equation}
\item Qubits rules:
\begin{equation}
\begin{gathered}
    \begin{tikzpicture}[basel={-0.5}]
   \inangarc{2}{(-0.5,0)}{90};
   \draw[markx={0},markx={0.8}] (-0.5,0) to (-0.25,0);
    \qubitl{(0,0)};
    \end{tikzpicture} \equiv\begin{tikzpicture}[basel={-.5}]]
    \draw[markx={0.5}] (0,0.5) to[bend left=90]  (0,-0.5) ;
\end{tikzpicture} , \quad   \begin{tikzpicture}[basel={-0.5}]
   \inangarc{2}{(-0.5,0)}{90};
   \draw[markx={0}] (-0.5,0) to (-0.25,0);
    \qubitl{(0,0)};
    \end{tikzpicture} \equiv\begin{tikzpicture}[basel={-.5}]]
    \draw[markx={0}] (-0.5,0.3) to (-0.25,0.3); 
    \draw[markx={0}] (-0.5,-0.3) to (-0.25,-0.3) ;
    \qubitl{(0,0.3)};
    \qubitl{(0,-0.3)};
\end{tikzpicture} , \quad \begin{tikzpicture}[basel={-1.5}]
  \qubitl{(0,0)};
  \draw[markx={0}](-0.5,0)to (-0.25,0);
  \draw[\rao](-1,0) to (-0.5,0);
  \draw (-0.8,0.3) node {$v$};
\end{tikzpicture} \equiv \begin{tikzpicture}[basel={-0.5}]
  \qubitl{(0,0)};
  \draw[markx={0}](-0.5,0)to (-0.25,0);\end{tikzpicture} , \quad \begin{tikzpicture}[basel={-1.5}]
  \qubitl{(0,0)};
  \draw[\rao](-0.75,0) to (-0.25,0);
  \draw (-0.5,0.3) node {$v$};
\end{tikzpicture} \equiv v\cdot \begin{tikzpicture}[basel={-0.5}]
  \qubitl{(0,0)};
  \draw[markx={0}](-0.5,0)to (-0.25,0);\end{tikzpicture} + \begin{tikzpicture}[basel={-0.5}]
  \qubitl{(0,0)};\end{tikzpicture}
  \\ 
\begin{tikzpicture}[basel={-1.5}]
  \qubitl{(0,0)};
  \draw[markx={1}](-1,0) to (-0.25,0);
  \ball{(-0.5,0)};
  \draw (-0.5,0.3) node {$w$};
\end{tikzpicture} \equiv w \cdot \begin{tikzpicture}[basel={-0.5}]
  \qubitl{(0,0)};
  \draw[markx={1}](-0.5,0) to (-0.25,0);
\end{tikzpicture} , \quad \begin{tikzpicture}[basel={-1.5}]
  \qubitl{(0,0)};
  \draw(-1,0) to (-0.25,0);
  \ball{(-0.5,0)};
  \draw (-0.5,0.3) node {$w$};
\end{tikzpicture} \equiv \frac{1}{w} \cdot \begin{tikzpicture}[basel={-0.5}]
  \qubitl{(0,0)};
  \draw(-0.5,0) to (-0.25,0);
\end{tikzpicture} .
    \label{eq:rule9}  
\end{gathered}
\end{equation}
\item 2 Qubits rules:
\begin{equation}
\begin{gathered}
  \begin{tikzpicture}[basel={-1.5},every node/.style={scale=0.6}]
            \draw[markx={1}](0,0) to (0.25,0);
            \draw(0.25,0) to[bend right=90] (0.75,0);
            \draw(0.25,0) to[bend left=90]  (0.75,0);
            \draw[markx={0}] (0.75,0) to (1,0); 
\ball{(0.5,0.15)};\draw (0.5,0.4) node{$v$};\end{tikzpicture} \equiv \sqrt{1+v^2} \cdot \begin{tikzpicture}[basel={-3}]
\draw (0,0) -- (1,0);
\ball{(0.5,0)}
\draw (0.5,0.5) node {$\frac{\sqrt{1+v^2}}{v}$};    
\end{tikzpicture}, \quad \begin{tikzpicture}[basel={-0.5},every node/.style={scale=0.6}]
            \draw[markx={1}](0,0) to (0.25,0);
            \draw(0.25,0) to[bend right=90] (0.75,0);
            \draw[markx={0.5}](0.25,0) to[bend left=90]  (0.75,0);
            \draw[markx={0}] (0.75,0) to (1,0); 
            \end{tikzpicture}\equiv \begin{tikzpicture}
                \draw[markx={0.5}](0,0) to (1,0);
            \end{tikzpicture}  , \quad 
     \begin{tikzpicture}[basel={-0.8}]
            \draw[markx={1}](0,0) to (0.25,0);
            \draw(0.25,0) to[bend right=90] (0.75,0);
            \draw[marko={0.5}](0.25,0) to[bend left=90]  (0.75,0);
            \draw[markx={0}] (0.75,0) to (1,0); 
            \end{tikzpicture} \equiv\begin{tikzpicture}[basel={-0.5}]
                \qubitl{(0,0)};
                \qubitr{(0.8,0)};
                \draw (-0.5,0) to (-0.25,0);
                 \draw(1.45,0) to (1.7,0);
            \end{tikzpicture}, \\
     \begin{tikzpicture}[basel={-0.8}]
            \draw[markx={1}](0,0) to (0.25,0);
            \draw[markx={0.5}](0.25,0) to[bend right=90] (1.25,0);
            \draw[markx={0.5}](0.25,0) to[bend left=90]  (1.25,0);
            \draw[markx={0}] (1.25,0) to (1.5,0); \ball{(1,0.3)};
            \draw (1,0.6) node{$v$};
            \end{tikzpicture} \equiv \left( \frac{1+v^2}{v}\right)\begin{tikzpicture}[basel={-0.5}]\qubitl{(0,0)};
                \qubitr{(0.8,0)};
                \draw[markx={0.5}] (-0.5,0) to (-0.25,0);
                 \draw[markx={0.5}](1.45,0) to (1.7,0);
            \end{tikzpicture}, \quad 
      \begin{tikzpicture}[basel={-0.8}]
            \draw[markx={1}](0,0) to (0.25,0);
            \draw[markx={0.5}](0.25,0) to[bend right=90] (1.25,0);
            \draw[markxo={0.5}{0.6}](0.25,0) to[bend left=90]  (1.25,0);
            \draw[markx={0}] (1.25,0) to (1.5,0); 
            \end{tikzpicture} \equiv \varnothing.
        \end{gathered}
         \label{eq:rule10}
\end{equation}
  \item Balls self-destruction: By using multiplication, movement, and pushing rules on balls, one can notice that they can be self-destroyed when going through an even number of elements ($\bullet$ and vertices):
    \begin{equation}
        \begin{tikzpicture}[basel={-0},every node/.style={scale=0.6}]
            \draw(0,0) to (0.5,0);
            \draw(0.5,0) to[bend right=90] (1.5,0);
            \draw[markx={0.5}](0.5,0) to[bend left=90]  (1.5,0);
            \draw (1.5,0) to (2,0); 
            \ball{(1,-0.3)};
            \draw (1,-0.5) node {$v$};
            \end{tikzpicture} \equiv \begin{tikzpicture}[basel={0.2},every node/.style={scale=0.6}]
            \draw(0,0) to (0.5,0);
            \draw(0.5,0) to[bend right=90] (1.5,0);
            \draw[markx={0.5}](0.5,0) to[bend left=90]  (1.5,0);
            \draw (1.5,0) to (2,0); 
            \ball{(0.7,-0.2)};
            \ball{(1.3,-0.2)};
            \draw (1.3,-0.5) node {$\sqrt{v}$};
             \draw (0.7,-0.5) node {$\sqrt{v}$};
            \end{tikzpicture} =\begin{tikzpicture}[basel={-0.4},every node/.style={scale=0.6}]
            \draw(0,0) to (0.5,0);
            \draw(0.5,0) to[bend right=90] (1.5,0);
            \draw[markx={0.5}](0.5,0) to[bend left=90]  (1.5,0);
            \draw (1.5,0) to (2,0); 
            \ball{(1,-0.3)};
            \ball{(0.7,0.2)};
            \draw (1,-0.5) node {$\sqrt{v}$};
             \draw (0.7,0.5) node {$1/\sqrt{v}$};
               \ball{(0.3,0)};
             \draw (0.3,0.3) node {$1/\sqrt{v}$};
    \end{tikzpicture}\equiv\begin{tikzpicture}[basel={-0.7},every node/.style={scale=0.6}]
            \draw(0,0) to (0.5,0);
            \draw(0.5,0) to[bend right=90] (1.5,0);
            \draw[markx={0.5}](0.5,0) to[bend left=90]  (1.5,0);
            \draw (1.5,0) to (2,0); 
            \ball{(1,-0.3)};
            \ball{(1.3,0.2)};
            \draw (1,-0.5) node {$\sqrt{v}$};
             \draw (1.3,0.5) node {$\sqrt{v}$};
             \ball{(0.3,0)};
             \draw (0.3,0.3) node {$1/\sqrt{v}$};
            \end{tikzpicture}=\begin{tikzpicture}[basel={0.2},every node/.style={scale=0.6}]
            \draw(0,0) to (0.5,0);
            \draw(0.5,0) to[bend right=90] (1.5,0);
            \draw[markx={0.5}](0.5,0) to[bend left=90]  (1.5,0);
            \draw (1.5,0) to (2,0); 
            \ball{(0.7,-0.2)};
            \ball{(1.3,-0.2)};
            \draw (1.3,-0.5) node {$1/\sqrt{v}$};
             \draw (0.7,-0.5) node {$\sqrt{v}$};
             \ball{(0.3,0)};
             \ball{(1.7,0)};
             \draw (0.3,0.3) node {$1/\sqrt{v}$};
              \draw (1.7,0.3) node {$1/\sqrt{v}$};
            \end{tikzpicture} \equiv\begin{tikzpicture}[basel={-0.6},every node/.style={scale=0.6}]
            \draw(0,0) to (0.5,0);
            \draw(0.5,0) to[bend right=90] (1.5,0);
            \draw[markx={0.5}](0.5,0) to[bend left=90]  (1.5,0);
            \draw (1.5,0) to (2,0); 
             \ball{(0.3,0)};
             \ball{(1.7,0)};
             \draw (0.3,0.3) node {$1/\sqrt{v}$};
              \draw (1.7,0.3) node {$1/\sqrt{v}$};
            \end{tikzpicture},
    \end{equation} 
    however, a register of balls when going through vertices must be kept.
 \end{enumerate}
We used this set of rules to study the construction for two, three, and four qubits, achieving graphs to build any SLOCC class. In \nameref{Appendix03} we show explicitly the use of the rules for these constructions. Here we, summarize the main results.
\subsubsection{Two Qubits}
For the two qubits case, there are two SLOCC classes, the separable class and the entangled class. Both can be obtained with the same graph but different parameters:
\begin{equation*}
     \begin{tikzpicture}[basel={-1}]
   \draw[markx={1}] (0,0) -- (0.5,0) ; 
   \draw [marko={0.5}](0.5,0)  to [bend left=50] (1.5,0) ;
   \draw  (1.5,0) to [bend left=50] (0.5,0) ;
   \draw [markx={0}] (1.5,0)-- (2,0);
\end{tikzpicture} = \begin{tikzpicture}[basel={-.5}]
    \qubitl{(0,0)}
    \qubitr{(0.8,0)}
    \draw(-0.5,0) to (-0.25,0);
      \draw(1.45,0) to (1.7,0);
\end{tikzpicture}  ,  \quad 
     \begin{tikzpicture}[basel={-1}]
   \draw[markx={1}] (0,0) -- (0.5,0) ; 
   \draw  (1.5,0) to [bend right=50] (0.5,0) ;
   \draw (1.5,0) to [bend left=50] (0.5,0) ;
   \draw[markx={0}]  (1.5,0)-- (2,0);
\end{tikzpicture} \cong \begin{tikzpicture}[basel={-.5}]
\draw (0,0) -- (1,0);   
\end{tikzpicture}
\end{equation*}
\subsubsection{Three Qubits}
\label{Threequbits}
Three qubit states are separated in $6$ SLOCC classes as shown in \nameref{Threequbitsclassification}. All can be obtained by modifications of the same graph. The completely separable state can be obtained as:
\begin{equation*}
\begin{tikzpicture}[basel={-.5}]
   \draw[markx={0.5},markx={0},markx={1}]  (-0.5,0) -- (-0.5,-1) ; 
   \draw (-0.5,-1) -- (-1,-1.5) ;
  \draw (-1,0.5)--(-0.5,0);
   \draw [markx={0.5},markx={0},markx={1}]  (0.5,-0.5)--(-0.5,0);
   \draw[markx={0.5}]  (-0.5,-1)--(0.5,-0.5);
   \draw  (0.5,-0.5)--(1,-0.5);
   \end{tikzpicture} =\begin{tikzpicture}[basel={-.5}]
    \qubitl{(0,0.2)}; 
    \qubitl{(0,-0.2)};
    \qubitr{(0.5,0)};
    \draw[markx={1}](-0.5,0.2)to (-0.25,0.2); 
   \draw[markx={1}](-0.5,-0.2)to (-0.25,-0.2); 
     \draw[markx={0}](1.15,0) to (1.4,0); \end{tikzpicture}.
   \end{equation*}
The classes $A-BC,B-AC,C-AB$ can be obtained as:
\begin{equation*}
\begin{tikzpicture}[basel={-.5}]
   \draw[markx={0.5},markx={0},markx={1}]  (-0.5,0) -- (-0.5,-1) ; 
   \draw (-0.5,-1) -- (-1,-1.5) ;
  \draw (-1,0.5)--(-0.5,0);
   \draw [markx={0},markx={1}]  (0.5,-0.5)--(-0.5,0);
   \draw[marko={0.5}](0.5,-0.5) -- (-0.5,-1);
   \draw  (0.5,-0.5)--(1,-0.5);
   \end{tikzpicture} =\begin{tikzpicture}[basel={-.5}] \draw[markx={0.5}](0,0.25) to [bend left=90](0,-0.25);\qubitr{(0.5,0)};
     \draw(1.15,0) to (1.4,0);
     \end{tikzpicture}.
   \end{equation*}
   The W class is the vertex on this construction, however, can also be obtained as:
   \begin{equation*}
\begin{tikzpicture}[basel={-.5}]
   \draw[markx={0.5},markx={0},markx={1}]  (-0.5,0) -- (-0.5,-1) ; 
   \draw (-0.5,-1) -- (-1,-1.5) ;
  \draw (-1,0.5)--(-0.5,0);
   \draw [markx={0},markx={1}]  (0.5,-0.5)--(-0.5,0);
   \draw[markx={0.5}](0.5,-0.5) -- (-0.5,-1);
   \draw  (0.5,-0.5)--(1,-0.5);
   \end{tikzpicture} =\begin{tikzpicture}[basel={-.5}] \draw[markx={1}](-0.5,0.5) to (0,0);
   \draw(-0.5,-0.5) to (0,0);
   \draw(0.5,0) to (0,0);   
     \end{tikzpicture}.
   \end{equation*}
Finally, the $GHZ$ class can be obtained as    
 \begin{equation}
\begin{tikzpicture}[basel={-.5}]
   \draw[markx={0},markx={1}]  (-0.5,0) -- (-0.5,-1) ; 
   \draw (-0.5,-1) -- (-1,-1.5) ;
  \draw (-1,0.5)--(-0.5,0);
   \draw [markx={0},markx={1}]  (0.5,-0.5)--(-0.5,0);
   \draw(0.5,-0.5) -- (-0.5,-1);
   \draw  (0.5,-0.5)--(1,-0.5);
   \end{tikzpicture} \cong \ket{GHZ}.
   \label{eq:triangleGHZ}
     \end{equation}
This last result was also obtained from the ZW perspective \cite{ZWGHZ}.
\section{SLOCC families -Graph equivalence for four qubits}
\label{FourQubitsVerst}
All SLOCC families for four qubits shown in Table \ref{table:fourqubitsclass} can be obtained when considering graphs with 6 $W$ vertices and 7 stitches. The SLOCC operations to go from the graph state to the representatives of each family are hard to find analytically for the families with more than one parameter; the correspondence shown here was obtained using the classification protocol shown in \cite{Holweck-class}, and the values of the parameters in the stitching are given to reproduce the same invariants as the representatives. The first SLOCC family is the $L_{0_{3\oplus \bar{1}}0_{3\oplus \bar{1}}}$ corresponding to the product state obtained from a qubit and a $GHZ$ state, one graph that can achieve it is:
\begin{equation*}
    \begin{tikzpicture}[basel={-.5}]
    \draw[markx={0.5},markx={0},markx={1}](0,0) to (1,0);
    \draw(1,0) to (1.5,0.5);
    \draw(1,0) to (1.5,-0.5);
    \draw(1.5,0.5) to (1.5,-0.5);
    \draw[markx={0}](1.5,0.5) to (1.75,0.75);
    \draw[markx={0}](1.5,-0.5) to (1.75,-0.75);
    \draw (0,0) to (0,0.25);
    \draw[markx={0.5}](-1,0)  to (0,0);
    \draw[marko={0.5},markx={0},markx={1}](-2,0) to [bend left=50](-1,0);
    \draw(-2,0) to [bend right=50](-1,0);
    \draw (-2,0) to (-2.25,0);
    \end{tikzpicture}\equiv \begin{tikzpicture}[basel={-.5}]
    \draw[markx={0.5},markx={0}](0,0) to (1,0);
    \draw[markx={0},markx={1}](1,0) to (1.5,0.5);
    \draw(1,0) to (1.5,-0.5);
    \draw[markx={1}](1.5,0.5) to (1.5,-0.5);
    \draw(1.5,0.5) to (1.75,0.75);
    \draw(1.5,-0.5) to (1.75,-0.75);
    \draw (0,0) to (0,0.25);
    \draw[markx={1}] (0,0) to (-0.25,0);
    \qubitr{(-0.9,0)};
    \qubitl{(-1.75,0)};
    \draw (-2,0) to (-2.25,0);
    \end{tikzpicture} \equiv 
    \begin{tikzpicture}[basel={-.5}]
    \draw (0,0) to (1,0);
    \draw[markx={1}](1,0) to (1.5,0.5);
    \draw[markx={0},markx={1}](1,0) to (1.5,-0.5);
    \draw(1.5,0.5) to (1.5,-0.5);
    \draw(1.5,0.5) to (1.75,0.75);
    \draw(1.5,-0.5) to (1.75,-0.75);
   \qubitl{(-0.75,0)};
    \draw(-1,0) to (-0.75,0);
    \end{tikzpicture} \cong \ket{L_{0_{3\oplus \bar{1}}0_{3\oplus \bar{1}}}}. 
\end{equation*}
Another three families can be obtained from the next graph:
\begin{equation*}
    \begin{tikzpicture}[basel={-.5}]
        \draw (0,0) to (-0.25,0);
        \draw[markx={0},markx={1}](0,0) to  (1,1) ;
         \draw(0,0) to  (1,-1) ;
          \draw (1,1) to  (1.5,0.5) ;
          \draw [markx={0},markx={1}](1,-1) to  (1.5,-0.5) ;
          \draw [markx={0},markx={1}](1.5,0.5) to (2,0)  ;
           \draw (1.5,-0.5) to (2,0)  ;
            \draw [\lac \rao](1.5,0.5) to (1.5,-0.5)  ;
            \draw (0.75,1.25) to (1,1);
            \draw (0.75,-1.25) to (1,-1);
            \draw (2.25,0) to (2,0);
    \end{tikzpicture}.
\end{equation*}
By changing the parameters of the arrows, two different families can be obtained:
\begin{equation*}
\begin{gathered}     \left(\tikz{\draw[\rao] (0,0) to (0.2,0) ;} =-1,\tikz{\draw[\rac] (0,0) to (0.2,0) ;} =(1,1)\right) \cong \ket{L_{0_{5\oplus\bar{3}}}} ,\\
\left(\tikz{\draw[\rao] (0,0) to (0.2,0) ;} =1,\tikz{\draw[\rac] (0,0) to (0.2,0) ;} =(1,1)\right) \cong \ket{L_{0_{7\oplus\bar{1}}}} .
\end{gathered}
\end{equation*}
One more family is obtained by using a $\bullet$ line:
\begin{equation*}
    \begin{tikzpicture}[basel=-1.5]
        \draw (0,0) to (-0.25,0);
        \draw[markx={0},markx={1}](0,0) to  (1,1) ;
         \draw(0,0) to  (1,-1) ;
          \draw [markx={0},markx={1}](1,1) to  (1.5,0.5) ;
          \draw[markx={0.5},markx={0},markx={1}](1,-1) to  (1.5,-0.5) ;
          \draw [markx={0},markx={1}](1.5,0.5) to (2,0)  ;
           \draw (1.5,-0.5) to (2,0)  ;
            \draw [\lac-](1.5,0.5) to (1.5,-0.5)  ;
            \draw (0.75,1.25) to (1,1);
            \draw (0.75,-1.25) to (1,-1);
            \draw (2.25,0) to (2,0);
            \draw (1.5,1) node {$-1$};
    \end{tikzpicture} \cong \ket{L_{a_4}}.
\end{equation*}
The remaining five SLOCC families can be obtained from the next graph:
\begin{equation*}
    \begin{tikzpicture}[basel={-.5}]
        \draw(0,0) to (1,0);
        \draw[markx={0},markx={1}] (0,0) to (0,-1);
        \draw (0,-1) to (1,-1);
        \draw[\lao-] (1,-1) to (2,0);
        \draw[\lac-] (1,0) to (2,-1);
        \draw (-0.25,0.25) to (0,0);
        \draw (0,-1) to (-0.25,-1.25);
        \draw (2,0) to (2.25,0.25);
        \draw[markx={0},markx={1}]  (1,0) to (2,0);
        \draw[markx={0},markx={1}]  (1,-1) to (2,-1);
        \draw (2,-1) to (2.25,-1.25);
    \end{tikzpicture},
\end{equation*}
The parameters for the nongeneric families are:
\begin{equation*}
\begin{gathered}     \left(\tikz{\draw[\rao] (0,0) to(0.2,0) ;} =0,\tikz{\draw[\rac] (0,0) to(0.2,0) ;} =(1,1)\right) \cong \frac{\sqrt{2}}{a} \ket{L_{a_20_{3\oplus\bar{1}}}} ,\\
\left(\tikz{\draw[\rao] (0,0) to(0.2,0) ;} =0,\tikz{\draw[\rac] (0,0) to(0.2,0) ;} =\left(\sqrt{\frac{a+b}{a-b}},\sqrt{\frac{a+b}{2a}}\right)\right) \cong \frac{\sqrt{2}}{\sqrt{a(a-b)}} \ket{L_{ab_3}} ,\\
\left(\tikz{\draw[\rao] (0,0) to(0.2,0) ;} =0,\tikz{\draw[\rac] (0,0) to(0.2,0) ;} =\left(\sqrt{\frac{a^2+b^2}{a^2 -b^2}},1\right)\right) \cong \frac{\sqrt{2}}{\sqrt{a^2-b^2}} \ket{L_{a_2b_2}},
 \\
\left(\tikz{\draw[\rao] (0,0) to(0.2,0) ;} =0,\tikz{\draw[\rac] (0,0) to(0.2,0) ;} =\left(\sqrt{\frac{c^2-ab}{c^2+ab}},\sqrt{\frac{c^2-a^2-b^2}{2(c^2+ab)}}\right)\right) \cong \frac{\sqrt{2}}{\sqrt{c^2+ab}} \ket{L_{abc_2}}.
\end{gathered}
\end{equation*}
The generic state can also be obtained, nevertheless, the parametrization is considerably more complicated, let's define the symmetric elements
\begin{equation*}
    s_1=(a+b+c+d), \quad s_2=(ab+ac+ad+bc+bd+cd), \quad s_3 = (abc+abd+acd+bcd), \quad s_4=abcd.
\end{equation*}
with this, let's define now $w_1^*,w_2^*$ as the solutions to the set
\begin{equation*}
    w_1^2+w_2^2 = \frac{s_1s_2}{s_1s_2-2s_3} \quad, \quad  w_1^2 w_2^2 =\frac{ 2 (s_1 s_2 s_3-s_1 ^2 s_4 -s_3^2)^2 } {(s_1 s_2 - 2 s_3)^3(s_1^3-2s_1 s_2 +4 s_3)},
\end{equation*}
and define
\begin{equation*}
v_2=\sqrt{\frac{s_1^3-2s_1 s_2 +4 s_3}{2 (s_1 s_2 -2 s_3)}} , f= \sqrt{\frac{2s_1}{s_1 s_2 -2 s_3}},
\end{equation*}
then, the generic state $G_{abcd}$ can be obtained as
\begin{equation*}
\left(\tikz{\draw[\rao] (0,0) to (0.2,0) ;} =w_1^*,\tikz{\draw[\rac] (0,0) to (0.2,0) ;} =\left(v_2,w_2^*\right)\right) \cong  f \ket{G_{abcd}}.
\end{equation*}
With this, we completed the 9 SLOCC families of Verstraette, and then, any 4 qubits state can be obtained from the graphs shown before. In the next chapter we will see how this multipartite qubit construction using $W$ states and bipartite states can be exploited to find explicit expressions for general Kronecker states and obtain a basis for Kronecker subspaces. Due to the completeness of \nameref{Schur-Weyl}  we can only ensure that any Kronecker subspace can be obtained if we are able to build any multipartite state, and here we shown how are these constructions explicitly done for the three and four qubits case.


 

==> FrontBackMatter/abstract_spanish.tex <==
\chapter*{Resumen}


==> FrontBackMatter/declaration.tex <==
\chapter*{Declaration}
I declare that the thesis has been composed by myself and that the work has not been
submitted for any other degree or professional qualification. I confirm that the work
submitted is my own, except where work which has formed part of jointly-authored
publications has been included. My contribution and those of the other authors to this
work have been explicitly indicated below. I confirm that appropriate credit has been
given within this thesis where reference has been made to the work of others.


==> FrontBackMatter/left_blank2.tex <==
\pagestyle{empty}
\begin{figure}
\includegraphics[scale=0.3]{Figures//G1.png}
\caption{Graphical representation of the 2.5 million of coefficients of a locally maximally entangled state of three parts in a Kronecker subspace}
\end{figure}



==> FrontBackMatter/notation.tex <==
\chapter*{Notation}
\begin{align*}
    U_\text{SB}(t) =& \text{system-bath unitary evolution} \\
    H_\text{SB} =& \text{system-bath Hamiltonian evolution} \\
    H_\text{int}, V =& \text{interaction hamiltonians} \\
    S^\alpha =& \text{system coupling operator} \\
    B^\alpha =& \text{bath coupling operator} \\
    \rho, \sigma =& \text{these are states} \\
    f,g =& \text{general functions} \\
    x,y,z =& \text{general variables} \\
    X,Y,Z =& \text{general matrices} \\
    \sigma^\text{x}_l,\sigma^\text{y}_l,\sigma^\text{z}_l =& \text{Pauli operators} \\
    t,t',\tau,t_1,t_2, =& \text{these are times} \\
    N,L =& \text{number of particles, spins} \\
    \Lambda, \mathcal{L},\mathcal{E}(t) =& \text{Lindblad and evolution operators} \\
    J_k, A_k =& \text{Jump operators, Kraus operators}
\end{align*}


\begin{align*}
    \Pi(E), P(E) =& \text{projectors and POVM elements} \\
    \mathcal{P,Q,I} =& \text{projections and identity map} \\
    \varepsilon_k, E_i, E =& \text{energies} \\
    r, R =& \text{random number and Random matrix} \\
    \lambda =& \text{weak-coupling constant} \\
    \mu,\sigma =& \text{mean and standard deviation} \\
    \mathcal{U}_\text{S},\mathcal{U}_\text{B} =& \text{system, bath internal energy} \\
    \dbar W, \dbar Q =& \text{differential work and heat} \\
    p(a,b), q(a,b) =& \text{probability distributions} \\
    \mathcal{S},\mathcal{S}_\text{vN}, \mathcal{S}_\text{B}, \mathcal{S}_\text{obs} =& \text{entropies} \\
    \gamma, \kappa =& \text{dissipation rates in extended and normal spaces} \\
    \mathcal{H} =& \text{Hilbert space} \\
    \mathcal{D}(\rho||\sigma) =& \text{relative entropy} \\
    \omega, \Omega  =& \text{system and bath frequencies} \\
    C(t),\hat{C}(\omega) =& \text{bath correlation function} \\
    \mathcal{T}_+ =& \text{time-ordering operator} \\
\end{align*}

==> FrontBackMatter/publications.tex <==
\chapter*{List of Publications}
\begin{refsection}[ownpubs]
    \small
    \nocite{aksin,angenendt,bertram,baez/article,sigfridsson}
    \printbibliography[heading=none]
\end{refsection}

